Reachability of Communicating Timed Processes

We study the reachability problem for communicating timed processes, both in discrete and dense time. Our model comprises automata with local timing constraints communicating over unbounded FIFO channels. Each automaton can only access its set of local clocks; all clocks evolve at the same rate. Our main contribution is a complete characterization of decidable and undecidable communication topologies, for both discrete and dense time. We also obtain complexity results, by showing that communicating timed processes are at least as hard as Petri nets; in the discrete time, we also show equivalence with Petri nets. Our results follow from mutual topology-preserving reductions between timed automata and (untimed) counter automata.

==> conclusions.tex <==

\section{Conclusions and future work}
\label{sec:conclusions}

We have studied the decidability and complexity of communicating timed processes.
In discrete time, we give a complete characterization of decidable topologies with emptiness tests,
as well as a tight connection with Petri nets in the test-free case.
%
In dense time, we prove decidability for polyforest test-free topologies,
and we generalize the undecidability results of \cite{Krcal:CAV:2006} to
arbitrary weakly-connected topologies containing two testable channels.
%
We leave open whether one can obtain, in the presence of emptiness tests,
the same characterization as in discrete time.
We conjecture that this is possible,
although the techniques used here do not seem to easily extend to deal with emptiness tests.
%
Finally, as another direction for future work one can study richer models
where processes are allowed to send timestamps or clocks along channels,
in the spirit of \cite{AbdullaAtigCederberg:12}.

\paragraph{Acknowledgements.}
We thank J\'er\^ome Leroux, Anca Muscholl, and Igor Walukiewicz for helpful discussions.


==> counter_automata.tex <==

%\vspace{-1ex}
\paragraph{Communicating counter automata.}
\label{sec:counter_automata}

A \emph{counter automaton} is a classical Minsky machine $\Cnt =
\tuple{L, L_I, L_F, A, X, \Delta}$ with finitely many locations $L$, initial
locations $L_I \subseteq L$, final locations $L_F \subseteq L$, alphabet of actions $A$,
finitely many counters in $X$, and transition rules $\Delta \subseteq L
\times A \times L$. Operations on a counter $x \in X$ are $\inc
x$ (increment), $\dec x$ (decrement) and $\ztest x$ (zero test).
Let $\Op(X)$ be the set of operations over counters in $X$.
We require that $A \supseteq \Op(X)$. % it is more natural the inclusion this way in the prose since A is the subject
%
As usual, the semantics is given as a labelled transition system
$\sem\Cnt = \tuple {S, S_I, S_F, A, \rightarrow}$ where $S = L \times
\Nat^X$, $S_I = L_I \times \{\lambda x . 0\}$, $S_F = L_F \times \{\lambda x . 0\}$,
and the transition relation $\rightarrow$ is defined as usual.
Notice that acceptance is with zero counters.

%\noindent
A \emph{system of communicating counter automata} is a system of communicating timed processes
$\Sys = \tuple{\Topo, M, \setD, (\sem{\Cnt^p})_{p \in P}}$
%(where $\Topo = \tuple{P, C, E}$ is a topology)
such that $\setD = \emptyset$ and each $\Cnt^p$ is a counter automaton.
By Definition~\ref{defn:sys_com_timed_proc}, this entails that each
counter automaton performs communicating actions in $A^p_{\textrm{\it com}}$.
Moreover, since the delay domain is empty,
they can only interact through the asynchronous exchange of messages.
%
%$\Sys$ is \emph{test-free} iff no counter automaton $\Cnt^p$ has a transition
%\greg{Do we still need this?}
%$\ctrans \ell a {\ell'}$ with $a = \ztest x$.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "m"
%%% End: 


==> introduction.tex <==

\section{Introduction}

\emph{Communicating automata} are a fundamental model for studying concurrent processes exchanging messages over unbounded channels
%(known as communicating finite-state machines in the seminal paper)
\cite{Pachl:TR:1982,Brand:1983:CFM:322374.322380}.
However, the model is Turing-powerful,
and even basic verification questions, like reachability, are undecidable.
To obtain decidability,
various restrictions have been considered,
%allowing only one kind of messages to be sent \cite{Peng:1992},
including making channels unreliable \cite{Abdulla:1996,chambart-p-2008-340-a} %Finkel:1996
%in the sense that messages can be lost after they are sent
or restricting to half-duplex communication \cite{Cece:2005}
(later generalized to mutex \cite{HeussnerLerouxMuschollSutre:2010}).
Decidability can also be obtained when restricting to executions satisfying additional restrictions,
such as bounded context-switching \cite{latorre-s-2008-299-a},
%there are finitely many phases, and in each phase exactly one process is allowed to read from at most one channel (writes are unrestricted)
or bounded channels.
%or even eagerness (i.e., a send must be immediately followed by its matching receive \cite{HeussnerLerouxMuschollSutre:2010}).
Finally, and this is the restriction that we consider here,
decidability is obtained by constraining the communication topology. % by forbidding directed cycles (including self-loops).
For communicating finite-state machines (CFSMs),
it is well-known that reachability is decidable if, and only if,
the topology is a polyforest \cite{Pachl:TR:1982,latorre-s-2008-299-a};
in this case, considering channels of size one suffices for deciding reachability.
%In fact, reachability remains decidable even when considering an additional operation of \emph{test of empty channel},
%which we use as a simpler primitive to model a certain \emph{urgent semantics} when reading the channels from \cite{Krcal:CAV:2006}

% SHORTENED below
%The reduction to $1$-bounded channels is not correct anymore when
%processes may also synchronize. For instance, a process may send an
%arbitrary number of messages $a$ before synchronizing on $\tau$ while
%the corresponding receiver waits synchronization on $\tau$ before
%starting to read messages. Such a system is not $1$-bounded, and even
%not existentially-bounded as all emissions must occur before the
%receptions take place. Synchronizations thus make CFSMs more
%expressive as the trace language $\{ (!a)^n \tau (?a)^n \, | \, n \in
%\mathbb{N} \}$ cannot be characterized by a CFSM with a polyforest
%topology, unless synchronizations (on $\tau$) are allowed.

On a parallel line of research,
\emph{timed automata} \cite{Alur:TCS:1994} have been extensively studied as a finite-state model of timed behaviours.
Recently, there have been several works bringing time into infinite-state models,
including \emph{timed Petri nets} \cite{TimedPetriNets:05,Abdulla:2001:TPN:647747.734218},
\emph{timed pushdown automata} \cite{AbdullaAtigStenmana:12},
and \emph{timed lossy channel systems} \cite{AbdullaAtigCederberg:12}.
%
In this paper, we study \emph{communicating timed processes} \cite{Krcal:CAV:2006},
where a finite number of timed automata synchronize over the elapsing of time
and communicate by exchanging messages over unbounded channels.
%
Note that, when processes can synchronize, runs cannot be re-ordered to have uniformly bounded channels (contrary to polyforest CFSMs).
For example, consider two communicating processes $p$ and $q$,
where $p$ can send to $q$ unboundedly many messages in the first time unit,
and $q$ can receive messages only after the first time unit has elapsed.
Clearly, all transmissions of $p$ have to occur before any reception by $q$,
which excludes the possibility of re-ordering the run into another one with bounded channels.

%(cf. Appendix~\ref{app:subsec:tick-expressivity}).
%
We significantly extend the results of \cite{Krcal:CAV:2006},
by giving a complete characterization of the decidability border of reachability properties w.r.t. the communication topology.
%
Quite surprisingly, we show that despite synchronization increases the expressive power of CFSMs,
the undecidability results of \cite{Krcal:CAV:2006} are not due to just synchronous time,
but to an additional synchronization facility called \emph{urgency} (cf. below).
Our study comprises both dense and discrete time.

%\vspace{-2ex}
\paragraph{Dense time: Communicating timed automata.}

%We also consider the dense-time model, i.e., classical timed automata \cite{Alur:TCS:1994}.
%Communicating timed automata with emptiness tests have been already considered in \cite{Krcal:CAV:2006}.
%Since discrete time can be modeled inside dense time,
%all our undecidability results on discrete time immediately transfer to the dense-time case.
%In particular, when considering $\alpha = 2$ counters and $\beta = 2$ zero tests,
%we obtain the undecidability results from \cite{Krcal:CAV:2006} for topologies $p \xrightarrow{} q \xrightarrow{} r$,
%as well as a new undecidability result for topologies $p \xrightarrow{} q \xleftarrow{} r$.
%
%However, for decidability results we do not allow emptiness tests,
%which allows us tackle arbitrary topologies. %as opposed to A --> B of \cite{Krcal:CAV:2006}
%We show that, when the only channel actions allowed are transmissions and receptions,
%we can reduce dense time to discrete time (in the polyforest architecture),
%and transfer the decidability results from the discrete-time case.
%In particular, we vastly generalize the decidability of \cite{Krcal:CAV:2006} from a simple 2-processes topology,
%to arbitrary polyforests.
%Moreover, we also solve an open problem from \cite{Krcal:CAV:2006}
%showing that systems with no emptiness test are decidable,
%thus two emptiness tests are necessary for undecidability.

%We consider a model of distributed time where each process has a local set of (private) clocks,
%and all clocks progress at the same rate.
Our main result is a complete characterization of the decidability frontier for communicating timed automata:
We show that reachability is decidable if, and only if,
the communication topology is a polyforest.
%which is the same characterization as for untimed CFSMs.
Thus, adding time does not change the decidability frontier w.r.t. CFSMs.
However, the complexity worsens:
From our results it follows that communicating timed automata
are at least as hard as Petri nets.%
\footnote{And probably exponentially worse, due to a blow-up when translating from dense to discrete time.}

Our decidability results generalize those of \cite{Krcal:CAV:2006}
over the standard semantics for communicating automata.
In the same work, also undecidability results are presented.
However, they rely on an alternative \emph{urgent semantics},
where, if a message can be received,
then all internal actions are disabled:
This provides an extra means of synchronization,
which makes already the very simple topology $p \xrightarrow{} q \xrightarrow{} r$ undecidable \cite{Krcal:CAV:2006}.
We show that, without urgency, this topology remains decidable.

Here, we do not consider urgency directly,
but we rather model it by introducing an additional \emph{emptiness test} operation on channels
on the side of the receiver.
This allows us to discuss topologies where emptiness tests (i.e., urgency) are restricted to certain components.
We show that, with emptiness tests,
not only the topology $p \xrightarrow{} q \xrightarrow{} r$ is undecidable, as in \cite{Krcal:CAV:2006},
but also $p \xrightarrow{} q \xleftarrow{} r$ and $p \xleftarrow{} q \xrightarrow{} r$.
Thus, we complete the undecidability picture for dense time.

All our results for dense time follow from a mutual, topology-preserving reduction to a discrete-time model
(discussed below).
Over polyforest topologies, we reduce from dense to discrete time when no channel can be tested for emptiness.
Over arbitrary topologies, we reduce from discrete to dense time, even in the presence of emptiness tests.
While the latter is immediate,
the former is obtained via a \emph{Rescheduling Lemma} for dense-time timed automata which is interesting on its own,
allowing us to schedule processes in fixed time-slots
where senders are always executed before receivers.
%We prove that it is always possible to reschedule any run of a timed automaton s.t.
%the fractional part of any non-integral time point falls somewhere in a fixed interval inside $(0;1)$.
%In this way, we ensure that a sender is always scheduled before a receiver
%(thus transmissions occur before receptions)
%by assigning a fixed disjoint time-slot to each process.
%A finite partitioning of $(0;1)$ suffices since,
%in a polyforest,
%there are no mutual dependencies.

%\vspace{-2ex}
\paragraph{Discrete time: Communicating tick automata.}

We provide a detailed analysis of communication in the discrete-time
model, where actions can only happen at integer time points.  As a
model of discrete time, we consider \emph{communicating tick
  automata}, where the flow of time is represented by an explicit tick
action: A process evolves from one time unit to the next by performing a tick action,
forcing all the other processes to perform a tick as well;
%\footnote{Ticks can be also seen as a form of global rendezvous synchronization.}
%In this way, the local time always agrees with the common global time.
all the other actions are asynchronous.
This model of discrete-time is called \emph{tick automata} in \cite{Gruber:DLT:2005},
which is related to the \emph{fictitious-time} model of \cite{Alur:TCS:1994}.
%to \emph{timed process language} \cite{Hennessy:Timed:1995},
%and to \emph{discrete-time process algebra} \cite{Baeten:Timed:2004}.%time unit delay operator

We provide a complete characterization of decidable and undecidable topologies for communicating tick automata:
%(cf. Theorem~\ref{thm:tick_decidability}).
We show that reachability is decidable if, and only if, the topology is a polyforest (like for CFSMs),
and, additionally, each weakly-connected component can test at most one channel for emptiness.
%
Our results follow from topology-preserving mutual reductions between communicating tick automata and counter automata.
As a consequence of the structure of our reductions,
we show that channels and counters are mutually expressible,
and similarly for emptiness tests and zero tests.
This allows us to also obtain complexity results for communicating tick automata:
We show that reachability in a system of communicating tick automata over a weakly-connected topology
has the same complexity as reachability in Petri nets.%
\footnote{The latter problem is known to be EXPSPACE-hard \cite{Lipton:1976},
and finding an upper bound is a long-standing open problem.}

%Let us say that a system of communicating tick automata is of type $(\alpha,\beta)$
%iff there are $\alpha$ channels, $\beta \leq \alpha$ of which can be tested for emptiness,
%and let us say that a counter automaton is of type $(\alpha,\beta)$
%iff there are $\alpha$ counters, $\beta \leq \alpha$ of which can be tested for zero.
%
%We show that, for a given system of $(\alpha,\beta)$-communicating tick automata,
%over an arbitrary connected topology (i.e., possibly with loops),
%we can build an equivalent system of $(\alpha,\beta)$-communicating counter automata
%\emph{over the same topology}.
%Intuitively, we replace explicit synchronization between sender and receiver by exchanging tick messages,
%using counters to keep track of the desynchronization%
%\footnote{This is reminiscent of a similar idea from \cite{Krcal:CAV:2006}};
%the correctness of emptiness tests is enforced with zero tests on counters.
%This provides decidability results (and upper bounds on the complexity),
%since reachability is decidable for communicating counter automata \cite{HeussnerLerouxMuschollSutre:2010}.

%Conversely, from a non-communicating $(\alpha, \beta)$-counter automaton,
%we build an equivalent system of $(\alpha, \beta)$-communicating tick automata
%(over a restricted topology).
%This provides undecidability of our model already when there are two channels which can both be tested for emptiness.

%\vspace{-2ex}
\paragraph{Related work.}

%Tick actions can be seen as a form of rendezvous synchronization.
%It is shown in \cite{Ramalingam:2000} that pushdown automata with many rendezvous actions are undecidable.
%(We show in the appendix that having one unbounded channel and two rendezvous actions brings about undecidability.)

Apart from \cite{Krcal:CAV:2006},
%The work closest to our setting is certainly \cite{Krcal:CAV:2006},
%(as we have already mentioned above),
%where communicating timed automata have been defined for the first time.
communication in a dense-time scenario has also been studied in \cite{Chandrasekaran:2006,AkshayGastinMukundKumar:2010,Akshay:2007}.
In particular, \cite{Chandrasekaran:2006}
proposes timed message sequence charts as the semantics of communicating timed automata,
and studies the scenario matching problem
where timing constraints can be specified on local processes,
later extended to also include send/receive pairs \cite{AkshayGastinMukundKumar:2010}. % which is typical in the context of MSCs.
Communicating event-clock automata,
a strict subclass of timed automata,
are studied in \cite{Akshay:2007}
where, instead of considering the decidability frontier w.r.t. the communication topology,
it is shown, among other results, that reachability is decidable for arbitrary topologies over existentially-bounded channels.
%
A crucial difference w.r.t. our work is that we do not put any restriction on the channels,
and we consider full timed automata.
%
In a distributed setting, the model of global time we have chosen is not the only possible.
In particular, \cite{Akshay:CONCUR:2008} studies decidability of networks of (non-communicating) timed asynchronous automata
in an alternative setting where each automaton has a local drift w.r.t. global time.
%They show that, while deciding whether there exists a local drift to reach a given configuration is decidable,
%the dual universal question is undecidable.
%
In the discrete-time setting, we mention the work \cite{Ibarra:2003},
which generalizes communicating tick automata to a loosely synchronous setting,
where local times, though different, can differ at most by a given bound.
While \cite{Ibarra:2003} shows decidability for a restricted two-processes topology,
we characterize decidability for arbitrary topologies.

%As source of infinity perpendicular to time,
%\greg{To gain space, we could drop this paragraph.}
%communicating processes with a local stack have been studied in
%\cite{latorre-s-2008-299-a,HeussnerLerouxMuschollSutre:2010}.
%Finally, we mention \cite{chambart-p-2008-340-a} as a work similar in spirit to ours,
%where decidability is studied for topologies of reliable, as well as unreliable channels.

%\todo[inline]{Don't know what to do with the following references:	
%	\cite{Asarin:CONCUR:1998} related to Lemma~\ref{lem:discretization-ta} (particularly the Lemma~2)????
%	\cite{Abdulla:LMCS:2010} sampled semantics of timed automata.
%	\cite{Krcal:CONCUR:2004} correctness of time-triggered automata vs. timed automata.
%}

%\vspace{-2ex}
\paragraph{Outline.}

In Sec.~\ref{sec:preliminaries} we introduce general notation;
in particular, we define communicating timed processes,
which allow us to uniformly model communication in both the discrete and dense time.
In Sec.~\ref{sec:tick_automata} we study the decidability and complexity for communicating tick automata (discrete time),
while in Sec.~\ref{sec:untiming} we deal with communicating timed automata (dense time).
Finally, Sec.~\ref{sec:conclusions} ends the paper with future work.
Full proofs are given in the appendix.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "m"
%%% End: 


==> timed_automata_def.tex <==

%\vspace{-2ex}
\paragraph{Communicating timed automata.}
\label{sec:timed_automata}

A \emph{timed automaton} $\TA = \tuple{L, L_I, L_F, X, \Sigma, \Delta}$
is defined by a finite set of locations $L$ with initial
locations $L_I \subseteq L$ and final locations $L_F \subseteq L$, a
finite set of \emph{clocks} $X$, a finite alphabet $\Sigma$ and a
finite set $\Delta$ of transitions rules $(\ell, \sigma, g, R, \ell')$
where $\ell, \ell' \in L$, $\sigma \in \Sigma$, the guard $g$ is a
conjunction of constraints $x \# c$ for $x \in X$, $\# \in \{ <, \le,
=, \ge, > \}$ and $c \in \Nat$, and $R \subseteq X$ is a set of clocks to reset.

% Clock variables in $X$ are interpreted in $\setRpos$ by a \emph{clock valuation} $v \in \setRpos^X$.
%
The semantics of $\TA$ is given by the timed process
$\STA = \tuple{S, S_I, S_F, A, \rightarrow}$, where
$S = L \times \setRpos^X$, $S_I = L_I \times \{\lambda x.\, 0\}$,
$S_F = L_F \times \{\lambda x.\, 0\}$,
$A = \Sigma \cup \setRpos$ is the set of actions, and there is a
transition $(\ell,v) \xra{d} (\ell, v')$ if $d \in \setRpos$ and
$v'(x) = v(x) + d$ for every clock $x$, and $(\ell,v) \xra{\sigma}
(\ell',v')$ if there exists a rule $(\ell, \sigma, g, R, \ell') \in
\Delta$ such that $g$ is satisfied by $v$ (defined in the natural way)
and $v'(x) = 0$ when $x \in R$, $v'(x) = v(x)$ otherwise.
%
We decorate a path
$(\ell_0, u_0) \xra{a_0, t_0} (\ell_1,u_1) \xra{a_1, t_1} \cdots (a_n, u_n)$
in $\STA$ with additional \emph{timestamps}
%$t_i = \sum_{\substack{j = 0,\dots,i-1 \\ a_j = d_j \in \Rpos}} d_j$.
$t_i = \sum \setof {a_j} {j = 0, \dots, i-1 \textrm{ and } a_j \in \Rpos}$.
%
Note that we require cloks to be zero on accepting runs,
which simplifies a construction later.%
\footnote{
It can be implemented by duplicating final locations,
and by resetting all clocks when entering the new final locations.}
W.l.o.g. we do not consider location invariants in timed automata as they can be encoded in the guards;
reachability is preserved since acceptance with zero cloks forbids the elapse of time upon entering the last location of an accepting run.


%Observe that $\STA$ has transitions labeled by actions $\sigma$ and
%delays $d \in \setRpos$. W.l.o.g., we only consider paths in $\STA$ that are alternating
%sequences of delays and actions: $(\ell_0, v_0) \xra{d_1} (\ell_0,
%u_1) \xra{t_1, \sigma_1} (\ell_1, v_1) \xra{d_2} (\ell_1, u_2)
%\xra{t_2, \sigma_2} \cdots (\ell_n, v_n)$. For convenience, every
%action $\sigma_i$ is labeled by an additional \emph{timestamp} $t_i = \sum_{j =
%  1}^i d_j$. By convention, $t_0 = 0$.

A \emph{system of communicating timed automata} is a system of communicating timed processes
$\Sys = \tuple{\Topo, M, \setRpos, (\sem{\TA^p})_{p \in P}}$
%(with $\Topo = \tuple{P, C, E}$ a topology)
where each $\TA^p$ is a timed automaton.
%
Note that each timed automaton has access only to its local clocks.
%
By Definition~\ref{defn:sys_com_timed_proc}, each
timed automaton performs communicating actions in $A^p_{\textrm com}$
and synchronizes with all the other processes over delay actions in $\setRpos$.

% Let $\setRpos$ be the set of non-negative real numbers, and let $X$ be
% a set of clock variables that range over $\setRpos$.
% %
% A \emph{clock constraint} is a conjunction of constraints $x \# c$ for
% $x \in X$, $\# \in \{ <, \le, =, \ge, > \}$ and $c \in \Nat$, e.g. $(x
% \le 3 \land y > 0)$. Let $\CC(X)$ denote the set of clock constraints
% over $X$.
% %
% A \emph{clock valuation} is a function $v \, : \, X \to \setRpos$. Let
% $\setRpos^X$ denote the set of clock valuations. We write $v \sat
% \phi$ when $v$ satisfies $\phi \in \CC(X)$ with the natural semantics.
% %
% Let $v + \delta$ be the valuation that associates $v(x) + \delta$ to
% every clock $x$ and $\delta \in \setRpos$. For $R \subseteq X$, let $v
% \reset{R}$ be the valuation that sets $x$ to $0$ if $x \in R$, and
% remains unchanged otherwise.

% A \emph{timed automaton (TA)} is a tuple $\TA = \tuple{L, L_I, L_F, X,
%   \Sigma, E}$ where $L$ is a finite set of locations with initial
% locations $L_I \subseteq L$ and final locations $L_F \subseteq L$, $X$
% is a finite set of clocks, $\Sigma$ is a finite alphabet of actions,
% and $E \, \subseteq \, L \times \Sigma \times \CC(X) \times 2^X \times
% L$ is a finite set of transition rules $(l, \sigma, g, R, l')$ where
% $g$ is the \emph{guard}, and $R$ is the set of clocks that are
% \emph{reset} on the transition.
% %
% The semantics of $\TA$ is given by the timed process $\STA = \tuple{S,
%   I, F, A, \rightarrow}$ where $S = L \times \setRpos^X$ is the set of
% configurations with initial configurations $I = L_I \times \{\lambda
% x.\, 0\}$ and final configurations $F = L_F \times \setRpos^X$, $A =
% \Sigma \cup \setRpos$ is the set of actions, and the transitions are
% defined by $(l,v) \xra{\sigma} (l',v')$ if there exists a rule $(l,
% \sigma, g, R, l')$ such that $v \models g$ and $v' = v \reset{R}$, and
% $(l,v) \xra{\delta} (l, v + \delta)$ for all $\delta \in \setRpos$.

% Observe that w.l.o.g. we can assume that a path in $\STA$ is an
% alternating sequence of delays and actions, $(l_0, v_0) \xra{\delta_1}
% (l_0, u_1) \xra{\sigma_1} (l_1, v_1) \xra{\delta_2} (l_1, u_2)
% \xra{\sigma_2} \cdots (l_n, v_n)$. We decorate every action $\sigma_i$
% in the path with a \emph{timestamp} $t_i = \sum_{j = 1}^i \delta_j$,
% with $t_0 = 0$ by convention. Hence a path is a sequence: $(l_0, v_0)
% \xra{\delta_1} (l_0, u_1) \xra{t_1,\sigma_1} (l_1, v_1) \xra{\delta_2}
% (l_1, u_2) \xra{t_2,\sigma_2} \cdots (l_n, v_n)$.


% A \emph{system of communicating timed automata} is a system of
% communicating timed processes $\Sys = \tuple{\Topo, M, \setD,
%   (\sem{\TA^p})_{p \in P}}$ where $\setD = \setRpos$ and each $\TA^p$
% is a timed automaton.
% %
% By Definition~\ref{defn:sys_com_timed_proc}, this entails that each
% timed automaton performs communicating actions in $A^p_{\textrm com}$
% and synchronizes with all the other processes over delay actions in
% $\setRpos$.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "m"
%%% End: 

